DeRisk: An Effective Deep Learning Framework for Credit Risk Prediction over Real-World Financial Data

Despite the tremendous advances achieved over the past years by deep learning techniques, the latest risk prediction models for industrial applications still rely on highly handtuned stage-wised statistical learning tools, such as gradient boosting and random forest methods. Different from images or languages, real-world financial data are high-dimensional, sparse, noisy and extremely imbalanced, which makes deep neural network models particularly challenging to train and fragile in practice. In this work, we propose DeRisk, an effective deep learning risk prediction framework for credit risk prediction on real-world financial data. DeRisk is the first deep risk prediction model that outperforms statistical learning approaches deployed in our company's production system. We also perform extensive ablation studies on our method to present the most critical factors for the empirical success of DeRisk.

==> tex/9.Acknowledge.tex <==
\section{Conclusion}
In this work, we proposed an effective deep learning framework, \emph{DeRisk}, which utilizes both sequential and non-sequential features for credit risk prediction. We apply careful data pre-processing to obtain clean and useful data for deep models, use MLM to pre-train the sequential model, adopt weighted BCE loss and oversampling to deal with the data imbalance problem, and select generalizable and stable training labels for better performance. 
The overall performance of \emph{DeRisk} largely outperforms existing approaches on real-world financial data. 
%Compared with the existing approaches, \emph{DeRisk} achieves better results on both non-sequential and sequential data.

We remark that it is unnecessary that a more complicated network always performs better. In our analysis, every component of the training framework including data pre-processing and a carefully designed optimization process are all critical to making deep learning models perform well on a real-world financial application.
We hope our framework and analysis can bring insights for a wide range of important commercial applications and inspire future research on developing more powerful deep learning tools for real-world industrial data. 

%On the other hand, we notice that some traditional machine learning algorithms such as XGBoost have excellent model
%expansibility, and just adding the prediction score of the deep network into the training of XGBoost as a new feature may work well. We believe a promising direction of future work will be the combination of deep learning and traditional machine learning algorithms.

